Proof Repair across Type Equivalences

We describe a new approach to automatically repairing broken proofs in the Coq proof assistant in response to changes in types. Our approach combines a configurable proof term transformation with a decompiler from proof terms to tactic scripts. The proof term transformation implements transport across equivalences in a way that removes references to the old version of the changed type and does not rely on axioms beyond those Coq assumes. We have implemented this approach in PUMPKIN Pi, an extension to the PUMPKIN PATCH Coq plugin suite for proof repair. We demonstrate PUMPKIN Pi's flexibility on eight case studies, including supporting a benchmark from a user study, easing development with dependent types, porting functions and proofs between unary and binary numbers, and supporting an industrial proof engineer to interoperate between Coq and other verification tools more easily.

==> equiv2.tex <==
Inductive I :=(@\vspace{-0.04cm}@)
| A : I(@\vspace{-0.04cm}@)
| B : I.(@\vspace{-0.04cm}@)

Inductive J :=(@\vspace{-0.04cm}@)
| (@\codediff{makeJ}@) : (@\codediff{bool}@) $\rightarrow$ J.(@\vspace{-0.04cm}@)
$\phantom{hi}$(@\vspace{-0.04cm}@)



==> equivproof.tex <==
swap$\phantom{^{2}}$T (l : Old.list T) : New.list T :=(@\vspace{-0.04cm}@)
  Old.list_rect T (fun (l : Old.list T) => New.list T)(@\vspace{-0.04cm}@)
    New.nil(@\vspace{-0.04cm}@)
    (fun t _ (IHl : New.list T) => New.cons T t IHl)(@\vspace{-0.04cm}@)
    l.(@\vspace{-0.04cm}@)
(@\vspace{-0.14cm}@)
Lemma section: $\forall$ T (l : Old.list T),(@\vspace{-0.04cm}@)
  swap$^{-1}$ T (swap T l) = l.(@\vspace{-0.04cm}@)
Proof.(@\vspace{-0.04cm}@)
  intros T l. symmetry. induction l as [ |a l0 H].(@\vspace{-0.04cm}@)
  - auto.(@\vspace{-0.04cm}@)
  - simpl. rewrite $\leftarrow$ H. auto.(@\vspace{-0.04cm}@)
Qed.(@\vspace{-0.04cm}@)

swap$^{-1}$ T (l : New.list T) : Old.list T :=(@\vspace{-0.04cm}@)
  New.list_rect T (fun (l : New.list T) => Old.list T)(@\vspace{-0.04cm}@)
    (fun t _ (IHl : Old.list T) => Old.cons T t IHl)(@\vspace{-0.04cm}@)
    Old.nil(@\vspace{-0.04cm}@)
    l.(@\vspace{-0.04cm}@)
(@\vspace{-0.14cm}@)
Lemma retraction: $\forall$ T (l : New.list T),(@\vspace{-0.04cm}@)
  swap T (swap$^{-1}$ T l) = l.(@\vspace{-0.04cm}@)
Proof.(@\vspace{-0.04cm}@)
  intros T l. symmetry. induction l as [t l0 H| ].(@\vspace{-0.04cm}@)
  - simpl. rewrite $\leftarrow$ H. auto.(@\vspace{-0.04cm}@)
  - auto.(@\vspace{-0.04cm}@)
Qed.(@\vspace{-0.04cm}@)


==> listswap.tex <==
Inductive list (T : Type) : Type :=(@\vspace{-0.04cm}@)
| (@\codediff{nil}@) : list T(@\vspace{-0.04cm}@)
| (@\codediff{cons}@) :  T $\rightarrow$ list T $\rightarrow$ list T.(@\vspace{-0.04cm}@)

Inductive list (T : Type) : Type :=(@\vspace{-0.04cm}@)
| (@\codediff{cons}@) : T $\rightarrow$ list T $\rightarrow$ list T(@\vspace{-0.04cm}@)
| (@\codediff{nil}@) : list T.(@\vspace{-0.04cm}@)




==> listtovect.tex <==
Inductive list (T : Type) : Type :=(@\vspace{-0.04cm}@)
| nil : list T(@\vspace{-0.04cm}@)
| cons : T $\rightarrow$ list T $\rightarrow$ list T.(@\vspace{-0.04cm}@)

Inductive vector (T : Type) : (@\codediff{nat}@) $\rightarrow$ Type :=(@\vspace{-0.04cm}@)
| nil : vector T (@\codediff{O}@)(@\vspace{-0.04cm}@)
| cons : T $\hspace{-0.06cm}\rightarrow$ $\hspace{-0.06cm}\forall\hspace{-0.06cm}$ (@\codediff{(n : nat)}@), $\hspace{-0.06cm}$vector$\hspace{-0.06cm}$ T$\hspace{-0.06cm}$ (@\codediff{n}@) $\hspace{-0.06cm}\rightarrow\hspace{-0.06cm}$ vector $\hspace{-0.06cm}$T $\hspace{-0.06cm}$(@\codediff{(S n)}@).(@\vspace{-0.04cm}@)


==> nat.tex <==
Inductive nat : Set :=
| O : nat
| S : nat $\rightarrow$ nat.

Inductive pos_nat : Set :=
| (@\codediff{1}@) : pos_nat
| S : pos_nat -> pos_nat.




==> nattobin.tex <==
(@\vspace{-0.04cm}@)
(@\vspace{-0.04cm}@)
(@\vspace{-0.04cm}@)
(@\vspace{-0.04cm}@)
(@\vspace{-0.14cm}@)
Inductive nat :=(@\vspace{-0.04cm}@)
| O : nat(@\vspace{-0.04cm}@)
| S : nat $\rightarrow$ nat.(@\vspace{-0.04cm}@)

Inductive positive :=(@\vspace{-0.04cm}@)
| xI : positive  $\rightarrow$ positive(@\vspace{-0.04cm}@)
| xO : positive  $\rightarrow$ positive (@\vspace{-0.04cm}@)
| xH : positive.(@\vspace{-0.04cm}@)
(@\vspace{-0.14cm}@)
Inductive N :=(@\vspace{-0.04cm}@)
| N0 : N (@\vspace{-0.04cm}@)
| Npos : (@\codediff{positive}@) $\rightarrow$ N.(@\vspace{-0.04cm}@)


==> overviewproof.tex <==
Proof.(@\vspace{-0.04cm}@)
  intros x. induction x as [a l IHl|]; intro y0.(@\vspace{-0.04cm}@)
  - simpl. rewrite (IHl y0). simpl.(@\vspace{-0.04cm}@)
    rewrite (app_assoc (rev y0) (rev l) (a::[])). auto.(@\vspace{-0.04cm}@)
  - induction y0 as [a l IHl|].(@\vspace{-0.04cm}@)
    + simpl. rewrite (app_nil_r (rev l) (a::[])). auto.(@\vspace{-0.04cm}@)
    + auto.(@\vspace{-0.04cm}@)
Qed.


==> records.tex <==
Handshake :=(@\vspace{-0.04cm}@)
  seq 32 bool * seq 32 bool.(@\vspace{-0.04cm}@)
(@\phantom{\}.}@)(@\vspace{-0.04cm}@)
Connection :=(@\vspace{-0.04cm}@)
  bool * (seq 2 bool *(@\vspace{-0.04cm}@)
 (seq 8 bool * (Handshake *(@\vspace{-0.04cm}@)
 (bool * (bool *(@\vspace{-0.04cm}@)
 (seq 32 bool * (bool *(@\vspace{-0.04cm}@)
  bool))))))).(@\vspace{-0.04cm}@)
(@\phantom{\}.}@)

Record Handshake := (@\codediff{MkHandshake}@) {(@\vspace{-0.04cm}@)
  (@\codediff{handshakeType}@) : seq 32 bool; (@\codediff{messageNumber}@) : seq 32 bool(@\vspace{-0.04cm}@)
}.(@\vspace{-0.04cm}@)
Record Connection := (@\codediff{MkConnection}@) {(@\vspace{-0.04cm}@)
  (@\codediff{clientAuthFlag}@) : bool;  (@\hspace{0.04cm}@)  (@\codediff{corked}@) : seq 2 bool;(@\vspace{-0.04cm}@)
  (@\codediff{corkedIO}@) : seq 8 bool;     (@\codediff{handshake}@) : Handshake;(@\vspace{-0.04cm}@)
  (@\codediff{isCachingEnabled}@) : bool; (@\codediff{keyExchangeEPH}@) : bool;(@\vspace{-0.04cm}@)
  (@\codediff{mode}@) : seq 32 bool;      (@\hspace{0.03cm}@)  (@\codediff{resumeFromCache}@) : bool;(@\vspace{-0.04cm}@)
  (@\codediff{serverCanSendOCSP}@) : bool;(@\vspace{-0.04cm}@)
}.


==> replica.tex <==
Inductive Term : Set :=(@\vspace{-0.04cm}@)
| Var : Identifier $\rightarrow$ Term(@\vspace{-0.04cm}@)
| (@\codediff{Int}@) : Z $\rightarrow$ Term(@\vspace{-0.04cm}@)
| (@\codediff{Eq}@) : Term $\rightarrow$ Term $\rightarrow$ Term(@\vspace{-0.04cm}@)
| Plus : Term $\rightarrow$ Term $\rightarrow$ Term(@\vspace{-0.04cm}@)
| Times : Term $\rightarrow$ Term $\rightarrow$ Term(@\vspace{-0.04cm}@)
| Minus : Term $\rightarrow$ Term $\rightarrow$ Term(@\vspace{-0.04cm}@)
| Choose : Identifier $\rightarrow$ Term $\rightarrow$ Term.(@\vspace{-0.04cm}@)
(@\vspace{-0.18cm}@)
Inductive Term : Set :=(@\vspace{-0.04cm}@)
| Var : Identifier $\rightarrow$ Term(@\vspace{-0.04cm}@)
| (@\codediff{Bool}@) : Identifier $\rightarrow$ Term(@\vspace{-0.04cm}@)
| (@\codediff{Eq}@) : Term $\rightarrow$ Term $\rightarrow$ Term(@\vspace{-0.04cm}@)
| (@\codediff{Int}@) : Z $\rightarrow$ Term(@\vspace{-0.04cm}@)
| Plus : Term $\rightarrow$ Term $\rightarrow$ Term(@\vspace{-0.04cm}@)
| Times : Term $\rightarrow$ Term $\rightarrow$ Term(@\vspace{-0.04cm}@)
| Minus : Term $\rightarrow$ Term $\rightarrow$ Term(@\vspace{-0.04cm}@)
| Choose : Identifier $\rightarrow$ Term $\rightarrow$ Term.(@\vspace{-0.04cm}@)

